Shop The Look: Building a Large Scale Visual Shopping System at Pinterest

As online content becomes ever more visual, the demand for searching by visual queries grows correspondingly stronger. Shop The Look is an online shopping discovery service at Pinterest, leveraging visual search to enable users to find and buy products within an image. In this work, we provide a holistic view of how we built Shop The Look, a shopping oriented visual search system, along with lessons learned from addressing shopping needs. We discuss topics including core technology across object detection and visual embeddings, serving infrastructure for realtime inference, and data labeling methodology for training/evaluation data collection and human evaluation. The user-facing impacts of our system design choices are measured through offline evaluations, human relevance judgements, and online A/B experiments. The collective improvements amount to cumulative relative gains of over 160% in end-to-end human relevance judgements and over 80% in engagement. Shop The Look is deployed in production at Pinterest.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> label_collection_calibration.tex <==
\subsection{Labeler calibration process}
This was initially challenging because we weren't able to find an owner with the correct skillset in this calibration process.

\subsubsection{Engineer and Product Manager-owned}
At first, we divided ownership of the calibration process between the product manager (PM) and the engineer. The PM best knows the user requirements, while engineers best know the technical requirements and can set up labeling templates, generate labeling questions, perform post-labeling analysis, and generate visualizations. In this paradigm, the engineer and PM jointly wrote up training guides and handled calibration, iterating on the training guide and thinking through edge cases until label consistency and quality met our bar.

\begin{table}
\begin{center}
\begin{tabular}{l r}
\hline
Calibration Iteration & >=80\% Label Consistency Rate \\
\hline\hline
1 & 15\% \\
6 & 54\% \\
7 & 60\% \\
8 & 74\% \\
9 & 83\% \\
\hline
\end{tabular}
\end{center}
\caption{Comparison of label consistency across calibration iterations of the home decor end-to-end precision evaluation. >=80\% label consistency rate is defined as the percentage of labels with >=80\% labeler agreement. Label consistency was largely stagnant from iterations 1-6, but dramatically improved from iteration 7 onward, after bringing in a home decor domain expert.}
\label{tab:calibration_hd_template}
\vspace{-5mm}
\end{table}

\subsubsection{Domain expert and Product Manager-owned}
With the previous process, it was sometimes difficult for calibration to converge (defined as achieving sufficiently high label consistency and quality) due to complicated tasks. For example, we spent over 2 months calibrating our home decor end-to-end precision evaluation for relevance (Figure~\ref{fig:dtn_candgen_sofia_question_example}), but it still wasn't anywhere near converging. There were too many home decor categories, and it was challenging to define whether two products were similar based on criteria such as shape, color, material, prints/pattern for fabric, subject/theme for artwork, arrangement of components, design details, etc. This complexity led to a huge number of edge cases, which proved difficult for the engineer and PM to reason through without additional assistance.

To address this, we brought in a domain expert in home decor, who had greater insights into the different edge cases and complexities of the domain, to help with calibration. The domain expert and PM now co-owned the calibration process, jointly refining details in the training guide and reviewing labelers' incorrect answers, while the engineer was solely responsible for engineering work. The result was vastly increased calibration velocity -- label consistency for the home decor end-to-end precision evaluation rapidly increased after this change, as shown in Table~\ref{tab:calibration_hd_template} from iteration 7 onward, and calibration finally converged. In summary, we found that harnessing the proper domain expertise was crucial to successful labeler calibration.

%The lesson learned here was that although it makes sense for both PM and engineers to participate in this calibration process, It is a mismatch of skill set for the engineer, and it results in lost productivity and lower calibration velocity. Having area experts to focus on things that they are individually good at is a much better use of people's time.

%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.7\linewidth]{assets/home_decor_template.png}
%\end{center}
%\caption{Example home decor labeling template.}
%\label{fig:home_decor_template}
%\end{figure}

\subsubsection{Calibration drift}
Even after calibration for a particular task converges initially, labelers tend to gradually become uncalibrated again if they go a long time without working on that task. One potential reason is that they grow less familiar with the training guide and begin to use more subjective judgements as a result. To prevent this from happening for mission-critical tasks like relevance evaluations, which are an important factor in launch decisions, we set up weekly labeling jobs to monitor this calibration drift and to keep labelers calibrated. This enables our relevance evaluations to remain dependable over time.


==> main_experimental_results.tex <==
\section{Experimental Results}
\label{sec:experimental_results}

Our detection and embedding experiments are evaluated via offline evaluations, human relevance evaluations, and online user engagement A/B experiments. For brevity, we report results for selected evaluations -- detection work focused on home decor, and so is evaluated against home decor relevance, whereas embedding work focused on fashion, and so is evaluated against fashion relevance.  In practice, we find there is a positive correlation between gains in offline metrics and online metrics.

\input{detection_experiments.tex}

\input{embedding_experiments.tex}



%To evaluate the quality of the ``Scene Decomposition'' component, we perform both offline and online evaluations.
%The online ``A/B'' experiments measure the impact on user engagement metrics, and serve as the final ``stamp of approval'' prior to fully deploying a change.
%In practice, we find there is a positive correlation between gains in offline metrics and online metrics.

%\subsubsection{Offline Detection Evaluation}
%\label{subsubsec:detection_offline_eval}

%\subsubsection{Relevance Evaluation}
%\label{subsubsec:decomposition_relevance}

%\subsubsection{Online A/B Experiment}
%Finally, we measure the impact of each detection model release on Shop The Look user engagement metrics via an ``A/B'' experiment.
%Ideally, positive gains on our offline evaluation metrics will translate to gains on our online engagement metrics.
%As Table~\ref{tab:detection_ab} demonstrates, this is indeed the case.

















%Our embedding experiments are evaluated via offline evaluations, human relevance evaluations, and online user engagement A/B experiments.

%\subsubsection{Offline Evaluation}
%\label{subsubsec:embedding_offline_eval}


%\subsubsection{End-to-end human relevance evaluation}
%\label{subsubsec:embedding_relevance}



%\subsubsection{Online A/B experiment}

